Control-guided Communication: Efficient Resource Arbitration and Allocation in Multi-hop Wireless Control Systems

In future autonomous systems, wireless multi-hop communication is key to enable collaboration among distributed agents at low cost and high flexibility. When many agents need to transmit information over the same wireless network, communication becomes a shared and contested resource. Event-triggered and self-triggered control account for this by transmitting data only when needed, enabling significant energy savings. However, a solution that brings those benefits to multi-hop networks and can reallocate freed up bandwidth to additional agents or data sources is still missing. To fill this gap, we propose control-guided communication, a novel co-design approach for distributed self-triggered control over wireless multi-hop networks. The control system informs the communication system of its transmission demands ahead of time, and the communication system allocates resources accordingly. Experiments on a cyber-physical testbed show that multiple cart-poles can be synchronized over wireless, while serving other traffic when resources are available, or saving energy. These experiments are the first to demonstrate and evaluate distributed self-triggered control over low-power multi-hop wireless networks at update rates of tens of milliseconds.

==> content/relWork.tex <==
% !TEX root = ../root.tex

\section{Related Work}
\label{sec:relWork}

Feedback control over wireless networks has received considerable attention, see for instance~\cite{mager2019feedback} for an overview. 
In~\cite{mager2019feedback}, the first solution for fast feedback control over multi-hop wireless networks was proposed, however, communication occurred in a periodic fashion.

STC is one possibility of limiting the amount of communication in control systems.
While a large body of work on STC exists~\cite{VeMaFu03,WaLe09,MaAnTa10}, the integration of STC with wireless system designs has rarely been considered.
Works that consider such an integration and evaluate their work through real experiments are collected in \tabref{tab:rel_work}.
None of them considers the combination of fast update intervals and multi-hop networks that we are targeting and that defines a crucial design point for future cyber-physical systems.
Moreover, the ability to reallocate unused resources to serve other traffic is only demonstrated in~\cite{araujo2011self,Araujo2014}, but for single-hop networks and for the control of a double tank process, requiring slow update intervals.
In contrast to these works, we showcase, building on the recent work~\cite{mager2019feedback}, that we can do STC over multi-hop networks at fast update intervals, while being able to reallocate unused resources \emph{and} to save energy.

% The STC concept was originally proposed in~\cite{VeMaFu03} and further developed in~\cite{WaLe09,MaAnTa10,AnTa10}.
% These works consider remote control scenarios, where the plant states and the control commands need to be communicated over a network.
% Distributed self-triggered control has been addressed, for instance, in~\cite{dimarogonas2012distributed,hu2017output,tahir2015self}.
% None of the mentioned references considers the integration of STC and wireless communication protocols.
% 
% Practical implementations of STC over wireless networks have been presented in~\cite{heshmati2014self,santos2014adaptive}, but the freed resources remain unused.
% In~\cite{Araujo2014}, a STC implementation is shown where a network scheduler allocates additional traffic if possible.
% However, the approach is only applicable to single-hop wireless networks and considers a double-tank process with slow dynamics.
% The integration of a wireless multi-hop protocol with a STC design is presented in~\cite{ma2018efficient}.
% Different from our work, unused bandwidth cannot be rescheduled and the update intervals are on the order of seconds.

\begin{table}
\caption{Experimental evaluation of self-triggered control over wireless networks.}
\label{tab:rel_work}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Work & Distributed & Fast update & Multi- & Reallocation & Energy\\
& & intervals & hop& &savings\\
\hline
\cite{Araujo2014} & no & no & no & yes & yes \\
\cite{ma2018efficient} & no & no & yes & no & yes \\
\cite{heshmati2014self} & no & yes & no & no & yes \\
\cite{santos2014adaptive} & no & yes & no & no & no \\
\cite{santos2015aperiodic} & no & yes & no & no & no \\
\cite{araujo2011self} & no&no&no&yes&yes \\
\textbf{This} &yes&yes&yes&yes&yes\\
\hline
\end{tabular}
\end{center}
\end{table}
\db{\cite{santos2014adaptive} and \cite{santos2015aperiodic} is basically the same setup, \cite{santos2015aperiodic} is a bit more advanced. Maybe enough to cite the newer reference}
\db{Leave out distributed?}


==> tikz/Self_Trigger.tex <==
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\node[draw,rectangle,minimum width=5em,minimum height =
3em,align=center](process){Physical\\ System};
\node[draw,rectangle,minimum width=5em,minimum
height=3em,align=center,right=2em of
process,RoyalBlue](self){\textcolor{RoyalBlue}{Self}\\
\textcolor{RoyalBlue}{Trigger}}; 
\node[draw,rectangle,align = left, below right
= 1em and 2em of self.north east,minimum width=6.5em](packet){Packet};
\node[draw,rectangle,align=left,below=0em of
packet.south,anchor=north,minimum width=6.5em](content){ \:\textbullet \, Data\\
\:\textcolor{RawSienna}{\textbullet}  \textcolor{RawSienna}{Next trigger}};

% Network
\node[draw,rectangle, minimum height = 0.4pt,below = 3em of
process.south west,minimum width = 15em,inner sep = 0pt,anchor =
west](netw_1){}; \node[draw,rectangle,minimum height = 0.4pt,below = 1em of
netw_1,minimum width = 15em, inner sep = 0pt](netw_2){};
\node at ($(netw_1)!0.5!(netw_2)$){Wireless Network};

% Network Manager
\node[draw,rectangle,minimum width=5em,minimum
height=3em,align=center,below=3em of
netw_2.south](NM){Network\\
Manager}; 

% arrows
\draw[->,>=latex](process) -- (self);
\node at($(self)!0.5!(packet)$)(self-packet){};
\draw[->,>=latex,dashed,RoyalBlue](self) -| (self-packet |- netw_1);
\draw[->,dashed,RoyalBlue](self-packet|-netw_2) |- (NM); 
\draw[->](NM) -| node[pos=0.7,left]{Schedule} (netw_2-|process);
\draw[-> ](netw_1-|process) -- (process);
\end{tikzpicture}


==> tikz/commVSperf.tex <==
\begin{tikzpicture} 

\begin{axis}[%
width=0.3\textwidth, 
height=0.125\textheight,
scale only axis,
xmin=0,
xmax=1, 
ymin=5,
ymax=15, 
xlabel = Normalized Communication $\mathcal{C}$,
ylabel = Error $\bar{e}$,
axis background/.style={fill=white},
legend style={at={( 0.4,0.99)}, anchor=north west},
%axis x line*=bottom,
%axis y line*=left,
xmajorgrids,
ymajorgrids, 
scaled ticks=false, 
tick label style={/pgf/number format/fixed,
 /pgf/number format/precision=4},
  ticklabel shift={.1cm},
]
\addplot[mark=asterisk, mark options={}, mark size=2.5000pt, draw=black,thick] 
table {%
1 6.553318246847312
0.50271950271950274 7.92743556212378
0.34547554871005005 8.125390028130218
0.27499065420560747 9.273392995949216
0.1852917665867306 12.589865045381526
};

\end{axis}
\end{tikzpicture}


==> tikz/model.tex <==
\tikzset{font=\scriptsize}
\begin{tikzpicture}
\node[draw,rectangle,minimum height = 2em,align = center](system1){Physical\\ System 1};
\node[draw,rectangle,below=0em of system1.north west, anchor = south west,inner sep=0,minimum width=0.8em, minimum height=0.8em](act1){{A}};
\node[draw,rectangle,below=0em of system1.north east, anchor = south east,inner sep=0,minimum width=0.8em, minimum height=0.8em](sens1){{S}};

\node[draw,rectangle, minimum height = 2em,align=center, right = 4.5em of system1](system2){Physical\\ System 2};
\node[draw,rectangle,below=0em of system2.north west, anchor = south west,inner sep=0,minimum width=0.8em, minimum height=0.8em](sens2){{S}};
\node[draw,rectangle,below=0em of system2.north east, anchor = south east,inner sep=0,minimum width=0.8em, minimum height=0.8em](act2){{A}};

\node[draw, rectangle, minimum width = 23em,above = 10em of $(system1)!0.5!(system2)$, minimum height = 1em](network){Wireless Network};

\node[draw, rectangle, above = 3em of system1,minimum width=4em](ctrl1){Ctrl 1};
\node[draw,rectangle,above=3em of system2,minimum width=4em](ctrl2){Ctrl 2};

\node[draw,rectangle,above = 3em of ctrl1.east, anchor=east](et1){ST1}; 
\node[draw,rectangle,above = 3em of ctrl2.west, anchor=west](et2){ST2}; 

\node[draw,rectangle, left = 2.5em of ctrl1,align=center](rem1){Remote\\ Sensor 1};
\node[draw,rectangle, right = 2.5em of ctrl2,align=center](rem2){Remote\\ Sensor 2};

\draw[->] (sens2)-- node[midway,right]{$y_2(k)$} (ctrl2.south-|sens2);
% \draw[->](sens2) |- (ctrl2);
\draw[->] (network.south-|act2)-- node[midway,right,align=center]{$u_2^1(k-1)$} (ctrl2.north-|act2);
\draw[->](ctrl1.south-|act1) -- node[midway, left]{$u_1(k)$} (act1);
\draw[->] (network.south-|act1)-- node[midway,left,align=center]{$u_1^2(k-1)$} (ctrl1.north-|act1);
\draw[->](ctrl2.south-|act2) -- node[midway,right]{$u_2(k)$}(act2);
\draw[->] (sens1)-- node[midway,left]{$y_1(k)$} (ctrl1.south-|sens1);
% \draw[->](sens1) |- (ctrl1);
\draw[->](ctrl1.north-|et1) -- node[midway,right]{$u_2^1(k)$} (et1);
\draw[->](ctrl2.north-|et2) -- node[midway,left]{$u_1^2(k)$} (et2);
\draw[->](et1) -- (network.south-|et1);
\draw[->](et2) -- (network.south-|et2);
\draw[->](rem1) -- (network.south -| rem1);
\draw[->](rem2) -- (network.south -| rem2);
\end{tikzpicture}

